Breakthroughs in Cool Star Physics with the Line Emission Mapper X-ray Probe

We outline some of the highlights of the scientific case for the advancement of stellar high energy physics using the Line Emission Mapper X-ray Probe ({\it LEM}). The key to advancements with LEM lie in its large effective area -- up to 100 times that of the {\it Chandra} MEG -- and 1~eV spectral resolution. The large effective area opens up for the first time the ability to study time-dependent phenomena on their natural timescales at high resolution, such as flares and coronal mass ejections, and also opens the sky to much fainter targets than available to {\it Chandra} or {\it XMM-Newton}.

==> Exo_refs-archive.tex <==
{\small

\noindent %\bibitem[Airapetian et al.(2016)]{Airapetian et al.(2016)} 
Airapetian, V.~S., Glocer, A., Gronoff, G., H{\'e}brard, E., \& Danchi, W.\ 2016, Nature Geoscience, 9, 452\\

\noindent %\bibitem[Bhardwaj et al.(2007)]{Bhardwaj et al.(2007)}
 Bhardwaj, A., et al.\ 2007, Planetary and Space Science, 55, 1135\\

\noindent %\bibitem[Cravens, Robertson, \& Snowden(2001)]{Cravens et al.(2001)} 
Cravens, T.~E., Robertson, I.~P., \& Snowden, S.~L.\ 2001, \jgr, 106, 24883 \\

\noindent %\bibitem[Cuntz, Saar, \& Musielak(2000)]{Cuntz et al.(2000)} 
Cuntz, M., Saar, S.~H., \& Musielak, Z.~E.\ 2000, \apjl, 533, L151\\

\noindent %\bibitem[Dong et al.(2018)]{Dong et al.(2018)} D
Dong, C.~F., Jin, M., Lingam, M., Airapetian, V. S., Ma, Y. J., van der Holst, B.\ 2018, Proc. Natl. Acad. Sci., 115, 260\\

\noindent %\bibitem[Ehrenreich et al.(2015)]{Ehrenreich et al.(2015)} 
Ehrenreich, D., et al.\ 2015, \nat, 522, 459 \\

\noindent %\bibitem[Erkaev et al.(2007)]{Erkaev et al.(2007)}
 Erkaev, N.~V., Kulikov, Y.~N., Lammer, H., Selsis, F., Langmayr, D., Jaritz, G.~F., \& Biernat, H.~K.\ 2007, \aap, 472, 329 \\

\noindent%\bibitem[Fossati et al.(2010)]{Fossati et al.(2010)} 
Fossati, L., et al.\ 2010, \apjl, 714, L222 \\

\noindent%\bibitem[Fulton \& Petigura(2018)]{Fulton et al.(2018)} 
Fulton, B.~J., \& Petigura, E.~A.\ 2018, \aj, 156, 264\\

\noindent%\bibitem[Gillon et al.(2017)]{Gillon et al.(2017)} 
Gillon, M., et al.\ 2017, \nat, 542, 456 \\

\noindent%\bibitem[Guedel(2007)]{Guedel(2007)}
 G{\"u}del, M.\ 2007, Living Reviews in Solar Physics, 4, 3 \\

\noindent%\bibitem[Iro \& Deming(2010)]{Iro et al.(2010)} 
Iro, N., \& Deming, L.~D.\ 2010, \apj, 712, 218 \\

\noindent%\bibitem[Kashyap, Drake, \& Saar(2008)]{Kashyap et al.(2008)} 
Kashyap, V.~L., Drake, J.~J., \& Saar, S.~H.\ 2008, \apj, 687, 1339\\

\noindent%\bibitem[Kulow et al.(2014)]{Kulow et al.(2014)} 
Kulow, J.~R., France, K., Linsky, J., \& Loyd, R.~O.~P.\ 2014, \apj, 786, 132 \\

\noindent%\bibitem[Lalitha, Schmitt, \& Dash(2018)]{Lalitha et al.(2018)} 
Lalitha, S., Schmitt, J.~H.~M.~M., \& Dash, S.\ 2018, \mnras, 477, 808 \\

\noindent%\bibitem[Lammer et al.(2003)]{Lammer et al.(2003)} 
Lammer, H., Selsis, F., Ribas, I., Guinan, E.~F., Bauer, S.~J., \& Weiss, W.~W.\ 2003, \apjl, 598, L121 \\

\noindent%\bibitem[Lanza(2009)]{Lanza(2009)} 
Lanza, A.~F.\ 2009, \aap, 505, 339 \\

\noindent%\bibitem[Lanza(2012)]{Lanza(2012)}
 Lanza, A.~F.\ 2012, \aap, 544, A23 \\

\noindent%\bibitem[Lavie et al.(2017)]{Lavie et al.(2017)} 
Lavie, B., et al.\ 2017,  \aap, 605, L7 \\

\noindent%\bibitem[Lecavelier des Etangs et al.(2012)]{Lecavelier des Etangs et al.(2012)}
 Lecavelier des Etangs, A., et al.\ 2012, \aap, 543, L4 \\

\noindent%\bibitem[Lingam et al.(2018)]{Lingam et al.(2018)} 
Lingam, M., Dong, C. F., Fang, X. H., Jakosky, B. M., Loeb, A.\ 2018, \apj, 853, 10 \\

\noindent%\bibitem[Linsky et al.(2010)]{Linsky et al.(2010)}
 Linsky, J.~L., Yang, H., France, K., Froning, C.~S., Green, J.~C., Stocke, J.~T., \& Osterman, S.~N.\ 2010, \apj, 717, 1291 \\

\noindent%\bibitem[Llama \& Shkolnik(2015)]{Llama et al.(2015)}
 Llama, J., \& Shkolnik, E.~L.\ 2015, \apj, 802, 41 \\
 
\noindent%\bibitem[Lopez \& Fortney(2013)]{Lopez et al.(2013)}
Lopez, E.~D., \& Fortney, J.~J.\ 2013, \apj, 776, 2 \\

\noindent%\bibitem[Maggio et al.(2015)]{Maggio et al.(2015)} 
Maggio, A., et al.\ 2015, \apjl, 811, L2 \\

\noindent%\bibitem[Miller et al.(2015)]{Miller et al.(2015)} 
Miller, B.~P., Gallo, E., Wright, J.~T., \& Pearson, E.~G.\ 2015, \apj, 799, 163 \\

\noindent%\bibitem[Murray-Clay, Chiang, \& Murray(2009)]{Murray-Clay et al.(2009)} 
Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 \\

\noindent%\bibitem[Owen \& Wu(2017)]{Owen et al.(2017)} 
Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 \\

\noindent%\bibitem[Owen \& Lai(2018)]{Owen et al.(2018)} 
Owen, J.~E., \& Lai, D.\ 2018, \mnras, 479, 5012 \\

\noindent%\bibitem[Penz, Micela,  \& Lammer(2008)]{Penz et al.(2008)} 
Penz, T., Micela, G., \& Lammer, H.\ 2008, \aap, 477, 309 \\

\noindent%\bibitem[Pillitteri et al.(2011)]{Pillitteri et al.(2011)} 
Pillitteri, I., G{\"u}nther, H.~M., Wolk, S.~J., Kashyap, V.~L., \& Cohen, O.\ 2011, \apjl, 741, L18 \\

\noindent%\bibitem[Pillitteri et al.(2014)]{Pillitteri et al.(2014)} 
Pillitteri, I., Wolk, S.~J., Lopez-Santiago, J., G{\"u}nther, H.~M., Sciortino, S., Cohen, O., Kashyap, V., \& Drake, J.~J.\ 2014, \apj, 785, 145 \\

\noindent%\bibitem[Poppenhaeger, Schmitt, \& Wolk(2013)]{Poppenhaeger et al.(2013)} 
Poppenhaeger, K., Schmitt, J.~H.~M.~M., \& Wolk, S.~J.\ 2013, \apj, 773, 62 \\

\noindent%\bibitem[Poppenhaeger \& Wolk(2014)]{Poppenhaeger et al.(2014)} 
Poppenhaeger, K., \& Wolk, S.~J.\ 2014, \aap, 565, L1 \\

\noindent%\bibitem[Sanz-Forcada et al.(2010)]{Sanz-Forcada et al.(2010)} 
Sanz-Forcada, J., Ribas, I., Micela, G., Pollock, A.~M.~T., Garc{\'{\i}}a-{\'A}lvarez, D., Solano, E., \& Eiroa, C.\ 2010, \aap, 511, L8 \\

\noindent%\bibitem[Tian et al.(2005)]{Tian et al.(2005)}
 Tian, F., Toon, O.~B., Pavlov, A.~A., \& De Sterck, H.\ 2005, Science, 308, 1014 \\

\noindent%\bibitem[Vidal-Madjar et al.(2003)]{Vidal-Madjar et al.(2003)} 
Vidal-Madjar, A., Lecavelier des Etangs, A., D{\'e}sert, J.-M., Ballester, G.~E., Ferlet, R., H{\'e}brard, G., \& Mayor, M.\ 2003, \nat, 422, 143\\

\noindent%\bibitem[Wood et al.(2018)]{Wood et al.(2018)} 
Wood, B.~E., Laming, J.~M., Warren, H.~P., \& Poppenhaeger, K.\ 2018, \apj, 862, 66 \\

\noindent%\bibitem[Yelle(2004)]{Yelle(2004)} 
Yelle, R.~V.\ 2004, Icarus, 170, 167 \\
}
%\end{bibliograpghy)

==> Exo_refs.tex <==

%\bibitem[Airapetian et al.(2016)]{Airapetian et al.(2016)} 
Airapetian, V.~S., Glocer, A., Gronoff, G., H{\'e}brard, E., \& Danchi, W.\ 2016, Nature Geoscience, 9, 452

%\bibitem[Bhardwaj et al.(2007)]{Bhardwaj et al.(2007)}
 Bhardwaj, A., et al.\ 2007, Planetary and Space Science, 55, 1135

%\bibitem[Cravens, Robertson, \& Snowden(2001)]{Cravens et al.(2001)} 
Cravens, T.~E., Robertson, I.~P., \& Snowden, S.~L.\ 2001, \jgr, 106, 24883 

%\bibitem[Cuntz, Saar, \& Musielak(2000)]{Cuntz et al.(2000)} 
Cuntz, M., Saar, S.~H., \& Musielak, Z.~E.\ 2000, \apjl, 533, L151

\bibitem[Dong et al.(2018)]{Dong et al.(2018)} Dong, C.~F., Jin, M., Lingam, M., Airapetian, V. S., Ma, Y. J., van der Holst, B.\ 2018, Proc. Natl. Acad. Sci., 115, 260

\bibitem[Ehrenreich et al.(2015)]{Ehrenreich et al.(2015)} Ehrenreich, D., 
et al.\ 2015, \nat, 522, 459 

\bibitem[Erkaev et al.(2007)]{Erkaev et al.(2007)} Erkaev, N.~V., Kulikov, Y.~N., Lammer, H., Selsis, F., Langmayr, D., Jaritz, G.~F., \& Biernat, H.~K.\ 2007, \aap, 472, 329 

\bibitem[Fossati et al.(2010)]{Fossati et al.(2010)} Fossati, L., et al.\ 2010, \apjl, 714, L222 

\bibitem[Fulton \& Petigura(2018)]{Fulton et al.(2018)} Fulton, B.~J., \& Petigura, E.~A.\ 2018, \aj, 156, 264

\bibitem[Gillon et al.(2017)]{Gillon et al.(2017)} Gillon, M., et al.\ 2017, \nat, 542, 456 

\bibitem[Guedel(2007)]{Guedel(2007)} G{\"u}del, M.\ 2007, Living Reviews in Solar Physics, 4, 3 

\bibitem[Iro \& Deming(2010)]{Iro et al.(2010)} Iro, N., \& Deming, L.~D.\ 2010, \apj, 712, 218 

\bibitem[Kashyap, Drake, \& Saar(2008)]{Kashyap et al.(2008)} Kashyap, V.~L., Drake, J.~J., \& Saar, S.~H.\ 2008, \apj, 687, 

\bibitem[Kulow et al.(2014)]{Kulow et al.(2014)} Kulow, J.~R., France, K., Linsky, J., \& Loyd, R.~O.~P.\ 2014, \apj, 786, 132 

\bibitem[Lalitha, Schmitt, \& Dash(2018)]{Lalitha et al.(2018)} Lalitha, S., Schmitt, J.~H.~M.~M., \& Dash, S.\ 2018, \mnras, 477, 808 

\bibitem[Lammer et al.(2003)]{Lammer et al.(2003)} Lammer, H., Selsis, F., Ribas, I., Guinan, E.~F., Bauer, S.~J., \& Weiss, W.~W.\ 2003, \apjl, 598, L121 

\bibitem[Lanza(2009)]{Lanza(2009)} Lanza, A.~F.\ 2009, \aap, 505, 339 

\bibitem[Lanza(2012)]{Lanza(2012)} Lanza, A.~F.\ 2012, \aap, 544, A23 

\bibitem[Lavie et al.(2017)]{Lavie et al.(2017)} Lavie, B., et al.\ 2017,  \aap, 605, L7 

\bibitem[Lecavelier des Etangs et al.(2012)]{Lecavelier des Etangs et al.(2012)} Lecavelier des Etangs, A., et al.\ 2012, \aap, 543, L4 

\bibitem[Lingam et al.(2018)]{Lingam et al.(2018)} Lingam, M., Dong, C. F., Fang, X. H., Jakosky, B. M., Loeb, A.\ 2018, \apj, 853, 10 

\bibitem[Linsky et al.(2010)]{Linsky et al.(2010)} Linsky, J.~L., Yang, H., France, K., Froning, C.~S., Green, J.~C., Stocke, J.~T., \& Osterman, S.~N.\ 2010, \apj, 717, 1291 

\bibitem[Llama \& Shkolnik(2015)]{Llama et al.(2015)} Llama, J., \& Shkolnik, E.~L.\ 2015, \apj, 802, 41 
\bibitem[Lopez \& Fortney(2013)]{Lopez et al.(2013)} Lopez, E.~D., \& Fortney, J.~J.\ 2013, \apj, 776, 2 

\bibitem[Maggio et al.(2015)]{Maggio et al.(2015)} Maggio, A., et al.\ 2015, \apjl, 811, L2 

\bibitem[Miller et al.(2015)]{Miller et al.(2015)} Miller, B.~P., Gallo, E., Wright, J.~T., \& Pearson, E.~G.\ 2015, \apj, 799, 163 

\bibitem[Murray-Clay, Chiang, \& Murray(2009)]{Murray-Clay et al.(2009)} Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 

\bibitem[Owen \& Wu(2017)]{Owen et al.(2017)} Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 

\bibitem[Owen \& Lai(2018)]{Owen et al.(2018)} Owen, J.~E., \& Lai, D.\ 2018, \mnras, 479, 5012 

\bibitem[Penz, Micela,  \& Lammer(2008)]{Penz et al.(2008)} Penz, T., Micela, G., \& Lammer, H.\ 2008, \aap, 477, 309 

\bibitem[Pillitteri et al.(2011)]{Pillitteri et al.(2011)} Pillitteri, I., G{\"u}nther, H.~M., Wolk, S.~J., Kashyap, V.~L., \& Cohen, O.\ 2011, \apjl, 741, L18 

\bibitem[Pillitteri et al.(2014)]{Pillitteri et al.(2014)} Pillitteri, I., Wolk, S.~J., Lopez-Santiago, J., G{\"u}nther, H.~M., Sciortino, S., Cohen, O., Kashyap, V., \& Drake, J.~J.\ 2014, \apj, 785, 145 

\bibitem[Poppenhaeger, Schmitt, \& Wolk(2013)]{Poppenhaeger et al.(2013)} Poppenhaeger, K., Schmitt, J.~H.~M.~M., \& Wolk, S.~J.\ 2013, \apj, 773, 62 

\bibitem[Poppenhaeger \& Wolk(2014)]{Poppenhaeger et al.(2014)} Poppenhaeger, K., \& Wolk, S.~J.\ 2014, \aap, 565, L1 

\bibitem[Sanz-Forcada et al.(2010)]{Sanz-Forcada et al.(2010)} Sanz-Forcada, J., Ribas, I., Micela, G., Pollock, A.~M.~T., Garc{\'{\i}}a-{\'A}lvarez, D., Solano, E., \& Eiroa, C.\ 2010, \aap, 511, L8 

\bibitem[Tian et al.(2005)]{Tian et al.(2005)} Tian, F., Toon, O.~B., Pavlov, A.~A., \& De Sterck, H.\ 2005, Science, 308, 1014 

\bibitem[Vidal-Madjar et al.(2003)]{Vidal-Madjar et al.(2003)} Vidal-Madjar, A., Lecavelier des Etangs, A., D{\'e}sert, J.-M., Ballester, G.~E., Ferlet, R., H{\'e}brard, G., \& Mayor, M.\ 2003, \nat, 422, 143

\bibitem[Wood et al.(2018)]{Wood et al.(2018)} Wood, B.~E., Laming, J.~M., Warren, H.~P., \& Poppenhaeger, K.\ 2018, \apj, 862, 66 

\bibitem[Yelle(2004)]{Yelle(2004)} Yelle, R.~V.\ 2004, \icarus, 170, 167 
\end{bibliograpghy)
